Two-Step Offline Preference-Based Reinforcement Learning with Constrained Actions

Preference-based reinforcement learning (PBRL) in the offline setting has succeeded greatly in industrial applications such as chatbots. A two-step learning framework where one applies a reinforcement learning step after a reward modeling step has been widely adopted for the problem. However, such a method faces challenges from the risk of reward hacking and the complexity of reinforcement learning. To overcome the challenge, our insight is that both challenges come from the state-actions not supported in the dataset. Such state-actions are unreliable and increase the complexity of the reinforcement learning problem at the second step. Based on the insight, we develop a novel two-step learning method called PRC: preference-based reinforcement learning with constrained actions. The high-level idea is to limit the reinforcement learning agent to optimize over a constrained action space that excludes the out-of-distribution state-actions. We empirically verify that our method has high learning efficiency on various datasets in robotic control environments.

==> figures/baseline.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=0.8\linewidth]{figures/naive.png}
% \vspace{-0.1in}
\caption{The blue line is the performance of the policies learned by the naive baseline method on the learned utility model (evaluated performance) and actual reward model (actual performance). The red line is the smoothed blue line.}
\label{fig:baseline}
\end{figure*}


==> figures/behavior.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=0.8\linewidth]{figures/pac.png}
% \vspace{-0.1in}
\caption{The blue line is the performance of the policies learned by the BR-PAC method on the learned utility model (evaluated performance) and actual reward model (actual performance). The red line is the smoothed blue line.}
\label{fig:behavior}
\end{figure*}

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/pac_2.png}
% % \vspace{-0.1in}
% \caption{Performance of the policies learned by the step method on the learned utility model and actual reward model.}
% \label{fig:behavior2}
% \end{figure}

==> figures/data.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=1.0\linewidth]{figures/_data.png}
% \vspace{-0.1in}
\caption{Training log of the BR-PAC method learned on Walker-medium datasets with different sizes}
\label{fig:data}
\end{figure*}

==> figures/full.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=1.0\linewidth]{figures/_full.png}
% \vspace{-0.1in}
\caption{Training log of the BR-PAC method learned on $8$ datasets.}
\label{fig:full}
\end{figure*}
